Query Efficient Weighted Stochastic Matching

In this paper, we study the weighted stochastic matching problem. Let $G=(V, E)$ be a given edge-weighted graph and let its realization $\mathcal{G}$ be a random subgraph of $G$ that includes each edge $e\in E$ independently with a known probability $p_e$. The goal in this problem is to pick a sparse subgraph $Q$ of $G$ without prior knowledge of $G$'s realization, such that the maximum weight matching among the realized edges of $Q$ (i.e. the subgraph $Q\cap \mathcal{G}$) in expectation approximates the maximum weight matching of the entire realization $\mathcal{G}$. Attaining any constant approximation ratio for this problem requires selecting a subgraph of max-degree $\Omega(1/p)$ where $p=\min_{e\in E} p_e$. On the positive side, there exists a $(1-\epsilon)$-approximation algorithm by Behnezhad and Derakhshan, albeit at the cost of max-degree having exponential dependence on $1/p$. Within the $\text{poly}(1/p)$ regime, however, the best-known algorithm achieves a $0.536$ approximation ratio due to Dughmi, Kalayci, and Patel improving over the $0.501$ approximation algorithm by Behnezhad, Farhadi, Hajiaghayi, and Reyhani. In this work, we present a 0.68 approximation algorithm with $O(1/p)$ queries per vertex, which is asymptotically tight. This is even an improvement over the best-known approximation ratio of $2/3$ for unweighted graphs within the $\text{poly}(1/p)$ regime due to Assadi and Bernstein. The $2/3$ approximation ratio is proven tight in the presence of a few correlated edges in $\mathcal{G}$, indicating that surpassing the $2/3$ barrier should rely on the independent realization of edges. Our analysis involves reducing the problem to designing a randomized matching algorithm on a given stochastic graph with some variance-bounding properties.

==> mainproof.tex <==
\section{Proof of the Main Theorem}\label{sec:main_proof}
In this section, we will put all the pieces together to prove our main theorem formally. In our proof, we will use an assumption about the size of the optimal solution due to ~\cite{behnezhad2020stochastic}. 
\begin{assumption}\cite{behnezhad2020stochastic}
\label{asuume:beh}
    We can assume without loss of generality that $|\textit{\opt}|= \O{n}$. Particularly, for any parameter $\xi\in (0,1)$ we can assume $|\opt|\geq  0.1\xi n$ at the cost of losing $\xi$ fraction of the  optimal solution.
\end{assumption}

Let us restate the main theorem for convenience.

\restatethm{\ref{thm:Themain}}{\thmmain{}}

% (direction and direction-intuition)
% \paragraph{Directions: }

% We use a fact that w.l.o.g. we can assume $\opt \geq \Omega(n)$. Intuitively, this will help eliminate the $2 \alpha n$ term we are losing in \cref{lem:fractionaldontdropmuch}. This argument is formalized below: 
\begin{proof}
We claim that the subgraph $Q$ outputted by  Algorithm~\ref{alg:query} indeed satisfies the statements of this lemma.  To prove this, we design another algorithm for finding a matching on $\mc{Q}$, the realized edges of $Q$. We then prove that it is a $0.681$-approximate matching in expectation. 

Let us consider the optimal solution $\opt$ and see how much of $\opt$ comes from the crucial edges $C$ versus the the non-crucial edges $N$. Let $\lambda$ be the fraction of $\opt$ on the crucial edges. We provide two schemes and show that the best of the two gives us the desired approximation ratio. One of these schemes is good when $\lambda$ is low, and one is good when $\lambda$ is high. 

The first scheme is to basically ignore the non-crucial edges and take a maximum matching of the  crucial edges of $\mc{Q}$. Due to Claim~\ref{claim:allcrucial}, the subgraph  $Q$ contains almost all the crucial edges. Particularly, it takes each one with probability at least $1- t\tau$. Plugging in the value of $\tau$ from table ~\ref{table:values} implies $\Pr[e\in Q]\geq 1- t(20p\epsilon^5\delta^2)$ for any $e\in C$. It is possible to pick a value for $t=O(1/p)$ to ensure 
\begin{equation}\label{eq:nkjjf}
    \Pr[e\in Q \mid e\in C]\geq 1-\epsilon/2.
\end{equation}
This implies that the first scheme achieves an  approximation ratio of at least $(1-\epsilon)\lambda$.

The second scheme we design works better when  $\lambda$ is smaller. We first run Algorithm~\ref{alg:Fu-modified} on the crucial edges in $\mc{Q}$ and find a matching $M_c$. Due to Lemma~\ref{lem:vertexindependent}, this algorithm is at least a $\frac{8}{15}$-approximation. Since each crucial edge may also be missed in $Q$ with probability at most $\epsilon/2$, then we have:
\begin{equation}\label{eq:Lnkjsjf}
    |M_c| \geq (1-\epsilon/2)\frac{8}{15}\lambda \opt.
\end{equation} We later show that due to the specific properties of $M_c$ we can construct a fractional matching $\bm{f}$ (using Algorithm~\ref{alg:fracmatching}) on the non-crucial edges whose both end-points are unmatched in $M_c$ with expected size at least 
$$\opt(1-\lambda)/(1+\sigma) - 2n\alpha \geq  \opt(1-\lambda)(1-\epsilon/3) -n\epsilon/5$$
The above inequality is due to Lemma~\ref{lem:fractionaldontdropmuch} and the fact that $(1-\lambda)$ fraction of the optimal solution comes from the non-crucial edges. Furthermore, Due to Lemma~\ref{lemm:integrhjk}, we know it is possible to round $\bm{f}$ and find an integral matching $M_n$ such that \begin{equation}\label{eq:kjfej}
    |M_n|\geq (1-\epsilon/10)(\opt(1-\lambda)(1-\epsilon/3) -n\epsilon/5)\geq\opt (1-\epsilon/2)\lambda -n\epsilon/5.
\end{equation}
Combining \eqref{eq:kjfej} and \eqref{eq:Lnkjsjf} implies:
\begin{equation*}
    |M_n\cup M_c|\geq (1-\epsilon/2)\left(1-\frac{7}{15}\lambda\right)\opt-n\epsilon/5.
\end{equation*}
By Assumption~\ref{asuume:beh} we can assume $\opt\geq n\xi/10$ at the cost of losing $\xi$ fraction of the optimal solution. Hence:
\begin{equation*}
    |M_n\cup M_c|\geq \left(1-\epsilon/2)(1-\frac{7}{15}\lambda\right)\opt-2\opt\epsilon/\xi-\xi.
\end{equation*}
Let us pick $\epsilon=\xi^2$ and hide all the terms with  $\xi$ or $\epsilon$ multiplied in them in $f(\xi)$. In other words, 
\begin{equation*}
    |M_n\cup M_c|\geq \left(1-\frac{7}{15}\lambda-f(\xi)\right)\opt.
\end{equation*}
Now, taking the best of the  solutions found by our two schemes we get a matching with approximation ratio $$\max\left(1-\frac{7}{15}\lambda - f(\xi), \lambda(1-\xi^2)\right) \geq 0.6818-\max (f(\xi),\xi^2) .$$ By picking a small enough value for $\xi$ we can ensure $\min(f(\xi),\xi^2)\leq 0.0008$ hence we get  an approximation ratio of $0.681$ and complete the proof.

 % Furthermore, on the non-crucial edges, by \cref{lem:fractionaldontdropmuch} we have that it is a $\frac{1}{1 + \sigma}$ approximation ignoring the $2\alpha n$ term which we deal separately with \cref{asuume:beh}.



% \paragraph{Math: } Now, with all the directions and intuitions above, we can discuss the technical part of the proof. The exact approximation ratio $\gamma_1$ we are getting with the first approach is: 

% \begin{align*}
%     \gamma_1 & \geq  [M_C \cdot (1 - \varepsilon_c)  - 2\alpha n] + (1 - \varepsilon_n) \cdot M_N
%     \\ & \geq  \lambda (1 - \varepsilon_n)  + (1 - \lambda) (1 - \varepsilon_n) - 2\alpha n
% \end{align*}

% Where for the first line, the first term refers to crucial edges and the second term refers to non-crucial edges. For $\epsilon_c = \frac{\epsilon}{10}$ (see ) $\epsilon_n = \frac{}.$ (see ) 

% The second approach is that our algorithm just takes the non-crucial edges into account which because their contribution is $1 - \lambda$, we get:

% $$
% \gamma_1 \geq (1 - \lambda) (1 - \varepsilon_n) - 2\alpha n
% $$

% Putting the two approximation ratios discussed above, our algorithm can for any instance make the best decision. Hence our final approximation ratio $\Gamma$, will be: 

% $$
% \Gamma \geq \min_{\lambda} \gamma_1(\lambda) - \gamma_2(\lambda) \geq 0.681
% $$

% For a small enough $\epsilon$.

% \mscomment{I can write the details of here too.}
% \\

% \mdcomment{(yes) / (no)}

\end{proof}

